Lower Bounds on Cross-Entropy Loss in the Presence of Test-time Adversaries

Understanding the fundamental limits of robust supervised learning has emerged as a problem of immense interest, from both practical and theoretical standpoints. In particular, it is critical to determine classifier-agnostic bounds on the training loss to establish when learning is possible. In this paper, we determine optimal lower bounds on the cross-entropy loss in the presence of test-time adversaries, along with the corresponding optimal classification outputs. Our formulation of the bound as a solution to an optimization problem is general enough to encompass any loss function depending on soft classifier outputs. We also propose and provide a proof of correctness for a bespoke algorithm to compute this lower bound efficiently, allowing us to determine lower bounds for multiple practical datasets of interest. We use our lower bounds as a diagnostic tool to determine the effectiveness of current robust training methods and find a gap from optimality at larger budgets. Finally, we investigate the possibility of using of optimal classification outputs as soft labels to empirically improve robust training.

==> plots/3_7_fmnist_l2_5000_loss_compare_.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4534.00,2266.00)%
    \gplgaddtomacro\gplbacktext{%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,440){\makebox(0,0)[r]{\strut{}\tiny 0}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,717){\makebox(0,0)[r]{\strut{}\tiny 10}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,994){\makebox(0,0)[r]{\strut{}\tiny 20}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,1271){\makebox(0,0)[r]{\strut{}\tiny 30}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,1548){\makebox(0,0)[r]{\strut{}\tiny 40}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,1825){\makebox(0,0)[r]{\strut{}\tiny 50}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(663,157){\makebox(0,0){\strut{}\tiny 2.5}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(1109,157){\makebox(0,0){\strut{}\tiny 3}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(1554,157){\makebox(0,0){\strut{}\tiny 3.5}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(1999,157){\makebox(0,0){\strut{}\tiny 4}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(2445,157){\makebox(0,0){\strut{}\tiny 4.5}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(2890,157){\makebox(0,0){\strut{}\tiny 5}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(3335,157){\makebox(0,0){\strut{}\tiny 5.5}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(3781,157){\makebox(0,0){\strut{}\tiny 6}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(58,1132){\rotatebox{-270}{\makebox(0,0){\strut{}\tiny{Classification loss}}}}%
      \put(2266,3){\makebox(0,0){\strut{}$\epsilon$}}%
      \csname LTb\endcsname%%
      \put(3847,727){\makebox(0,0)[r]{\strut{}\tiny{Minimum loss}}}%
      \csname LTb\endcsname%%
      \put(3847,595){\makebox(0,0)[r]{\strut{}\tiny{Hard labels}}}%
      \csname LTb\endcsname%%
      \put(3847,463){\makebox(0,0)[r]{\strut{}\tiny{Soft optimal labels}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={226.70bp},height={113.30bp}]{plots/3_7_fmnist_l2_5000_loss_compare}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/3_7_fmnist_l2_5000_loss_compare_resnet_test_.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4534.00,2266.00)%
    \gplgaddtomacro\gplbacktext{%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,440){\makebox(0,0)[r]{\strut{}\tiny 0}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,638){\makebox(0,0)[r]{\strut{}\tiny 0.1}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,836){\makebox(0,0)[r]{\strut{}\tiny 0.2}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,1034){\makebox(0,0)[r]{\strut{}\tiny 0.3}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,1231){\makebox(0,0)[r]{\strut{}\tiny 0.4}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,1429){\makebox(0,0)[r]{\strut{}\tiny 0.5}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,1627){\makebox(0,0)[r]{\strut{}\tiny 0.6}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,1825){\makebox(0,0)[r]{\strut{}\tiny 0.7}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(396,157){\makebox(0,0){\strut{}\tiny 2}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(864,157){\makebox(0,0){\strut{}\tiny 2.5}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(1331,157){\makebox(0,0){\strut{}\tiny 3}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(1799,157){\makebox(0,0){\strut{}\tiny 3.5}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(2267,157){\makebox(0,0){\strut{}\tiny 4}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(2734,157){\makebox(0,0){\strut{}\tiny 4.5}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(3202,157){\makebox(0,0){\strut{}\tiny 5}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(3669,157){\makebox(0,0){\strut{}\tiny 5.5}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(4137,157){\makebox(0,0){\strut{}\tiny 6}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(-74,1132){\rotatebox{-270}{\makebox(0,0){\strut{}\tiny{Cross-entropy loss}}}}%
      \put(2266,3){\makebox(0,0){\strut{}$\epsilon$}}%
      \csname LTb\endcsname%%
      \put(3983,953){\makebox(0,0)[r]{\strut{}\tiny{Hard labels}}}%
      \csname LTb\endcsname%%
      \put(3983,821){\makebox(0,0)[r]{\strut{}\tiny{TRADES ($\beta=1.0$)}}}%
      \csname LTb\endcsname%%
      \put(3983,689){\makebox(0,0)[r]{\strut{}\tiny{TRADES ($\beta=6.0$)}}}%
      \csname LTb\endcsname%%
      \put(3983,557){\makebox(0,0)[r]{\strut{}\tiny{Optimal soft}}}%
      \csname LTb\endcsname%%
      \put(3983,425){\makebox(0,0)[r]{\strut{}\tiny{Optimal clipped soft}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={226.70bp},height={113.30bp}]{plots/3_7_fmnist_l2_5000_loss_compare_resnet_test}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/3_7_mnist_l2_5000_loss_compare_.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4534.00,2266.00)%
    \gplgaddtomacro\gplbacktext{%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,440){\makebox(0,0)[r]{\strut{}\tiny 0}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,717){\makebox(0,0)[r]{\strut{}\tiny 10}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,994){\makebox(0,0)[r]{\strut{}\tiny 20}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,1271){\makebox(0,0)[r]{\strut{}\tiny 30}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,1548){\makebox(0,0)[r]{\strut{}\tiny 40}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,1825){\makebox(0,0)[r]{\strut{}\tiny 50}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(396,157){\makebox(0,0){\strut{}\tiny 3}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(1331,157){\makebox(0,0){\strut{}\tiny 3.5}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(2267,157){\makebox(0,0){\strut{}\tiny 4}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(3202,157){\makebox(0,0){\strut{}\tiny 4.5}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(4137,157){\makebox(0,0){\strut{}\tiny 5}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(58,1132){\rotatebox{-270}{\makebox(0,0){\strut{}\tiny{Classification loss}}}}%
      \put(2266,3){\makebox(0,0){\strut{}$\epsilon$}}%
      \csname LTb\endcsname%%
      \put(3847,727){\makebox(0,0)[r]{\strut{}\tiny{Minimum loss}}}%
      \csname LTb\endcsname%%
      \put(3847,595){\makebox(0,0)[r]{\strut{}\tiny{Hard labels}}}%
      \csname LTb\endcsname%%
      \put(3847,463){\makebox(0,0)[r]{\strut{}\tiny{Soft optimal labels}}}%
      \csname LTb\endcsname%%
      \put(3847,331){\makebox(0,0)[r]{\strut{}\tiny{trades}}}%
      \csname LTb\endcsname%%
      \put(3847,199){\makebox(0,0)[r]{\strut{}\tiny{trades, $\beta=6.0$}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={226.70bp},height={113.30bp}]{plots/3_7_mnist_l2_5000_loss_compare}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/3_7_mnist_l2_5000_loss_compare_resnet_test_.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4534.00,2266.00)%
    \gplgaddtomacro\gplbacktext{%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,440){\makebox(0,0)[r]{\strut{}\tiny 0}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,638){\makebox(0,0)[r]{\strut{}\tiny 0.1}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,836){\makebox(0,0)[r]{\strut{}\tiny 0.2}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,1034){\makebox(0,0)[r]{\strut{}\tiny 0.3}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,1231){\makebox(0,0)[r]{\strut{}\tiny 0.4}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,1429){\makebox(0,0)[r]{\strut{}\tiny 0.5}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,1627){\makebox(0,0)[r]{\strut{}\tiny 0.6}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(201,1825){\makebox(0,0)[r]{\strut{}\tiny 0.7}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(396,157){\makebox(0,0){\strut{}\tiny 2}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(1020,157){\makebox(0,0){\strut{}\tiny 2.5}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(1643,157){\makebox(0,0){\strut{}\tiny 3}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(2267,157){\makebox(0,0){\strut{}\tiny 3.5}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(2890,157){\makebox(0,0){\strut{}\tiny 4}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(3514,157){\makebox(0,0){\strut{}\tiny 4.5}}%
      \colorrgb{0.50,0.50,0.50}%%
      \put(4137,157){\makebox(0,0){\strut{}\tiny 5}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(-74,1132){\rotatebox{-270}{\makebox(0,0){\strut{}\tiny{$0-1$ loss}}}}%
      \put(2266,3){\makebox(0,0){\strut{}$\epsilon$}}%
      \csname LTb\endcsname%%
      \put(3983,953){\makebox(0,0)[r]{\strut{}\tiny{Hard labels}}}%
      \csname LTb\endcsname%%
      \put(3983,821){\makebox(0,0)[r]{\strut{}\tiny{TRADES ($\beta=1.0$)}}}%
      \csname LTb\endcsname%%
      \put(3983,689){\makebox(0,0)[r]{\strut{}\tiny{TRADES ($\beta=6.0$)}}}%
      \csname LTb\endcsname%%
      \put(3983,557){\makebox(0,0)[r]{\strut{}\tiny{Optimal soft}}}%
      \csname LTb\endcsname%%
      \put(3983,425){\makebox(0,0)[r]{\strut{}\tiny{Optimal clipped soft}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={226.70bp},height={113.30bp}]{plots/3_7_mnist_l2_5000_loss_compare_resnet_test}}%
    \gplfronttext
  \end{picture}%
\endgroup

